User-Relatedness and Community Structure in Social Interaction Networks

With social media and the according social and ubiquitous applications finding their way into everyday life, there is a rapidly growing amount of user generated content yielding explicit and implicit network structures. We consider social activities and phenomena as proxies for user relatedness. Such activities are represented in so-called social interaction networks or evidence networks, with different degrees of explicitness. We focus on evidence networks containing relations on users, which are represented by connections between individual nodes. Explicit interaction networks are then created by specific user actions, for example, when building a friend network. On the other hand, more implicit networks capture user traces or evidences of user actions as observed in Web portals, blogs, resource sharing systems, and many other social services. These implicit networks can be applied for a broad range of analysis methods instead of using expensive gold-standard information. In this paper, we analyze different properties of a set of networks in social media. We show that there are dependencies and correlations between the networks. These allow for drawing reciprocal conclusions concerning pairs of networks, based on the assessment of structural correlations and ranking interchangeability. Additionally, we show how these inter-network correlations can be used for assessing the results of structural analysis techniques, e.g., community mining methods.

==> tabs/correlations/bibsonomy.conductance.cor.tex <==
% latex.table(x = result.tau, file = paste(output.filename, ".cor",      sep = ""), dec = 3, table.env = FALSE) 
%
\begin{center}
\begin{tabular}{|l||c|c|c|c|c|c|} \hline
\multicolumn{1}{|l||}{/tmp/output.cor}&\multicolumn{1}{c|}{clickGraph}&\multicolumn{1}{c|}{copyGraph}&\multicolumn{1}{c|}{followerGraph}&\multicolumn{1}{c|}{friendGraph}&\multicolumn{1}{c|}{groupGraph}&\multicolumn{1}{c|}{visitGraph}\\ \hline
clickGraph&0.323&0.771&0.217&0.738&0.535&0.793\\ 
copyGraph&0.409&0.467&0.245&0.724&0.518&0.775\\ 
followerGraph&0.506&0.482&0.539&0.309&0.212&0.267\\ 
friendGraph&0.441&0.482&0.156&0.413&0.616&0.782\\ 
groupGraph&0.288&0.320&0.073&0.280&0.449&0.529\\ 
visitGraph&0.416&0.465&0.118&0.375&0.038&0.518\\ 
\hline
\end{tabular}
\end{center}


==> tabs/correlations/bibsonomy.conductance.p.tex <==
% latex.table(x = result.p, file = paste(output.filename, ".p",      sep = ""), dec = 3, table.env = FALSE) 
%
\begin{center}
\begin{tabular}{|l||c|c|c|c|c|c|} \hline
\multicolumn{1}{|l||}{/tmp/output.p}&\multicolumn{1}{c|}{clickGraph}&\multicolumn{1}{c|}{copyGraph}&\multicolumn{1}{c|}{followerGraph}&\multicolumn{1}{c|}{friendGraph}&\multicolumn{1}{c|}{groupGraph}&\multicolumn{1}{c|}{visitGraph}\\ \hline
clickGraph&0.000&0.000&0.000&0.000&0.000&0.000\\ 
copyGraph&0.000&0.000&0.000&0.000&0.000&0.000\\ 
followerGraph&0.000&0.000&0.000&0.000&0.000&0.000\\ 
friendGraph&0.000&0.000&0.000&0.000&0.000&0.000\\ 
groupGraph&0.000&0.000&0.000&0.000&0.000&0.000\\ 
visitGraph&0.000&0.000&0.000&0.000&0.004&0.000\\ 
\hline
\end{tabular}
\end{center}


==> tabs/correlations/bibsonomy.modularity.p.tex <==
% latex.table(x = result.p, file = paste(output.filename, ".p",      sep = ""), dec = 3, table.env = FALSE) 
%
\begin{center}
\begin{tabular}{|l||c|c|c|c|c|c|} \hline
\multicolumn{1}{|l||}{/tmp/output.p}&\multicolumn{1}{c|}{clickGraph}&\multicolumn{1}{c|}{copyGraph}&\multicolumn{1}{c|}{followerGraph}&\multicolumn{1}{c|}{friendGraph}&\multicolumn{1}{c|}{groupGraph}&\multicolumn{1}{c|}{visitGraph}\\ \hline
clickGraph&0.000&0.000&0.000&0.000&0.000&0.000\\ 
copyGraph&0.000&0.000&0.000&0.000&0.000&0.000\\ 
followerGraph&0.000&0.057&0.002&0.000&0.000&0.000\\ 
friendGraph&0.000&0.114&0.162&0.000&0.000&0.000\\ 
groupGraph&0.000&0.026&0.015&0.000&0.000&0.000\\ 
visitGraph&0.000&0.001&0.005&0.000&0.000&0.000\\ 
\hline
\end{tabular}
\end{center}


==> tabs/correlations/twitter.conductance.cor.tex <==
% latex.table(x = result.tau, file = paste(output.filename, ".cor",      sep = ""), dec = 3, table.env = FALSE) 
%
\begin{center}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|} \hline
\multicolumn{1}{|l||}{/tmp/output.cor}&\multicolumn{1}{c|}{follower}&\multicolumn{1}{c|}{11-17.RT\_red}&\multicolumn{1}{c|}{11-17.RT}&\multicolumn{1}{c|}{11-17.UM\_red}&\multicolumn{1}{c|}{11-17.UM}&\multicolumn{1}{c|}{RT\_red}&\multicolumn{1}{c|}{RT}&\multicolumn{1}{c|}{UM\_red}&\multicolumn{1}{c|}{UM}\\ \hline
follower&0.745&0.720&0.790&0.775&0.773&0.758&0.810&0.768&0.792\\ 
11-17.RT\_red&0.626&0.810&0.863&0.778&0.796&0.893&0.830&0.745&0.767\\ 
11-17.RT&0.643&0.780&0.807&0.828&0.857&0.874&0.916&0.804&0.842\\ 
11-17.UM\_red&0.683&0.731&0.772&0.767&0.864&0.804&0.836&0.886&0.845\\ 
11-17.UM&0.650&0.733&0.789&0.701&0.761&0.821&0.862&0.869&0.920\\ 
RT\_red&0.648&0.785&0.812&0.716&0.759&0.821&0.875&0.780&0.796\\ 
RT&0.667&0.762&0.806&0.717&0.737&0.782&0.822&0.840&0.871\\ 
UM\_red&0.690&0.688&0.753&0.725&0.728&0.694&0.758&0.773&0.867\\ 
UM&0.655&0.717&0.773&0.704&0.746&0.720&0.780&0.699&0.801\\ 
\hline
\end{tabular}
\end{center}


==> tabs/correlations/twitter.conductance.p.tex <==
% latex.table(x = result.p, file = paste(output.filename, ".p",      sep = ""), dec = 3, table.env = FALSE) 
%
\begin{center}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|} \hline
\multicolumn{1}{|l||}{/tmp/output.p}&\multicolumn{1}{c|}{follower}&\multicolumn{1}{c|}{11-17.RT\_red}&\multicolumn{1}{c|}{11-17.RT}&\multicolumn{1}{c|}{11-17.UM\_red}&\multicolumn{1}{c|}{11-17.UM}&\multicolumn{1}{c|}{RT\_red}&\multicolumn{1}{c|}{RT}&\multicolumn{1}{c|}{UM\_red}&\multicolumn{1}{c|}{UM}\\ \hline
follower&0&0&0&0&0&0&0&0&0\\ 
11-17.RT\_red&0&0&0&0&0&0&0&0&0\\ 
11-17.RT&0&0&0&0&0&0&0&0&0\\ 
11-17.UM\_red&0&0&0&0&0&0&0&0&0\\ 
11-17.UM&0&0&0&0&0&0&0&0&0\\ 
RT\_red&0&0&0&0&0&0&0&0&0\\ 
RT&0&0&0&0&0&0&0&0&0\\ 
UM\_red&0&0&0&0&0&0&0&0&0\\ 
UM&0&0&0&0&0&0&0&0&0\\ 
\hline
\end{tabular}
\end{center}


==> tabs/correlations/twitter.modularity.p.tex <==
% latex.table(x = result.p, file = paste(output.filename, ".p",      sep = ""), dec = 3, table.env = FALSE) 
%
\begin{center}
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|} \hline
\multicolumn{1}{|l||}{/tmp/output.p}&\multicolumn{1}{c|}{follower}&\multicolumn{1}{c|}{11-17.RT\_red}&\multicolumn{1}{c|}{11-17.RT}&\multicolumn{1}{c|}{11-17.UM\_red}&\multicolumn{1}{c|}{11-17.UM}&\multicolumn{1}{c|}{RT\_red}&\multicolumn{1}{c|}{RT}&\multicolumn{1}{c|}{UM\_red}&\multicolumn{1}{c|}{UM}\\ \hline
follower&0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000\\ 
11-17.RT\_red&0.000&0.247&0.000&0.000&0.000&0.000&0.000&0.000&0.000\\ 
11-17.RT&0.000&0.129&0.032&0.000&0.000&0.000&0.000&0.000&0.000\\ 
11-17.UM\_red&0.000&0.230&0.004&0.005&0.000&0.000&0.000&0.000&0.000\\ 
11-17.UM&0.000&0.154&0.020&0.055&0.005&0.000&0.000&0.000&0.000\\ 
RT\_red&0.000&0.000&0.000&0.000&0.000&0.003&0.000&0.000&0.000\\ 
RT&0.000&0.187&0.000&0.000&0.000&0.020&0.001&0.000&0.000\\ 
UM\_red&0.000&0.000&0.000&0.000&0.000&0.065&0.000&0.000&0.000\\ 
UM&0.000&0.083&0.000&0.000&0.000&0.046&0.000&0.000&0.000\\ 
\hline
\end{tabular}
\end{center}

